Towards Meaningful Statements in IR Evaluation. Mapping Evaluation Measures to Interval Scales

Recently, it was shown that most popular IR measures are not interval-scaled, implying that decades of experimental IR research used potentially improper methods, which may have produced questionable results. However, it was unclear if and to what extent these findings apply to actual evaluations and this opened a debate in the community with researchers standing on opposite positions about whether this should be considered an issue (or not) and to what extent. In this paper, we first give an introduction to the representational measurement theory explaining why certain operations and significance tests are permissible only with scales of a certain level. For that, we introduce the notion of meaningfulness specifying the conditions under which the truth (or falsity) of a statement is invariant under permissible transformations of a scale. Furthermore, we show how the recall base and the length of the run may make comparison and aggregation across topics problematic. Then we propose a straightforward and powerful approach for turning an evaluation measure into an interval scale, and describe an experimental evaluation of the differences between using the original measures and the interval-scaled ones. For all the regarded measures - namely Precision, Recall, Average Precision, (Normalized) Discounted Cumulative Gain, Rank-Biased Precision and Reciprocal Rank - we observe substantial effects, both on the order of average values and on the outcome of significance tests. For the latter, previously significant differences turn out to be insignificant, while insignificant ones become significant. The effect varies remarkably between the tests considered but overall, on average, we observed a 25% change in the decision about which systems are significantly different and which are not.

==> section/basic_results_old.tex <==
\section{Basic Results}
\label{sec:bas_res}

{\color{blue} Let us consider the three more common set-based measures, namely Precision, Recall and F-Measure.
It has been proven (see ...) that these measures are interval with respect to 
the same ordering amongst the runs,
once the length of the run and the Recall base are fixed values. 
If this assumption is 
violated, i.e. we consider together runs with different length and/or
different Recall base, this is no more true, i.e. the three measures are no more interval with respect to the same ordering. This can be seen simply proving 
that their values are no more related by an affine transformation.  
In this section we see that any of these three measure is interval 
even if we consider runs of different length and/or different Recall base.
The price to be paid is that now any of these measures are interval with respect to
a different ordering amongst the runs, and therefore they are no more related
by an affine transformation. The key to obtain this result is to consider the
measures for different length and/or Recall bases as the same measure expressed on  different unit of measurements. So, in order to consider them all together,
we first transform them into the same unit of measurement and the final measure is interval.}

\subsection{Precision}
Let us star by Precision. If r denotes a run of $N$ documents, Prec[r] 
is defined as the 
percentage of relevant documents among the retrieved ones, i.e.
\[
Prec[r]=\frac{1}{N} \sum_{i=1}^N r [i] \ .
\]
This means that the possible 
theoretical values it assumes are all the non negative rational numbers of the form $k/N$
where $k=0,1,\ldots, N$. In order to compare runs with different length and to perform a 
sound statistical analysis using these data, we have first to make these data homogeneous.
Assume for example that we have to consider the mean value of precision for the two
following runs: $r=[1,1,0]$ and $s=[1,1,0,0]$. Their lengths are equal to 3 and 4, respectively,
and the Lowest Common Multiple of these two values is 12. Is it possible to represent these two runs 
as runs of length 12 with the same precision scores of the original runs? The answer is yes and 
the transformed runs are, respectively, $\hat r=[1,1,1,1,1,1,1,1,0,0,0,0]$ and
$\hat s=[1,1,1,1,1,1,0,0,0,0,0,0]$.
These two runs are now evaluated by $Prec@12$ which is an interval measure and the statistical
analysis can be performed with no additional precautions.
In general we can proceed as follows: if we want to compare data coming from runs of different
lengths, namely $N_1, N_2, \ldots, N_m$, we first evaluate $\mathcal{N}$ the Lowest Common Multiple of these numbers 
and then represent each run as the equivalent run of this larger length. If for example a run of
length $N_1$ contains $k$ relevant documents, being its precision score equal to $k/N_1$, 
we transform it into the run of length $\mathcal{N}$ with $(k \mathcal{N})/N_1$ relevant documents.
Note that by the choice of $\mathcal{N}$, the number of relevant documents is still an integer value
and the new run has the same Precision of the former one, as desired.
In conclusion, we perform the statistical analysis considering the transformed runs and applying
to them the interval measure $Prec@\mathcal{N}$.
It is immediate to see that the same procedure works if we would like to consider all possible run's 
lengths up to a finite threshold $N$. In this case we can evaluate the the Lowest Common Multiple $\mathcal{N}$
of all the positive integers less or equal to $N$ and consider again the measure $Prec@\mathcal{N}$.
As a limit, if we do not restrict ourselves to a finite maximum length, we can represent any
run of finite length $N$ as an infinite sequence of $0$'s and $1$'s just making an infinite copy of the original one,
$\hat r=[r,r,r,r,\ldots]$. The new measure, that we can baptize 
$Prec@\infty$, is defined as
\[
Prec@\infty[\hat r]=\lim_{n\rightarrow\infty} Prec@n[\hat r]
\]
and it is immediate to prove that $Prec@\infty[\hat r]=Prec@N[r]$.
$Prec@\infty$ is a interval measure on $\mathbb{Q}\cap[0,1]$ and so again the statistical soundness of
the analysis of run of any possible length with the values of $Prec$ is saved.

\subsection{Recall}
The Recall measure depends on the recall base $RB$, which denotes the total number of relevant documents
available for a given topic.
We will denote this measure as $Recall(N,RB)$ and its definition is
\[
Recall(N,RB)[r]=\frac{1}{RB} \sum_{i=1}^N r [i]
\]
%where again $\hat r[i]$ denotes the relevance of the $i$-th document in the run $r$.
With respect to Precision, this measure from a pure theoretical point of view do not really depends
on the total length of the run, since its value does not change if we add to a run any number of
not relevant documents and move $N$ to this new bound. 
We have seen in the IEEE paper that, fixed the length of the runs to a given value $N$ and the value of recall base $RB$, 
$Recall(N,RB)$ is an interval measure. Indeed, $Recall(N,RB)=\frac{N}{RB} Prec@N$ and any linear transformation
of an interval measurement is itself interval.
But what happens if we would like to consider runs with different length and/or Recall bases?
As before done for Precision, we can find a unique space of runs \& Recall bases where embed all the runs and evaluate
them with a unique measure. The situation here is slightly more delicate than before: indeed we have to consider
two parameters, the length of the run and the Recall base. However, the first can be easily solved as follows:
given a set of runs that we have evaluated thanks to Recall, we take the length of the longest and transform the 
others to runs of the same length by adding a suitable number of not relevant document.
For example, taking $r=[1,1,0,0,0]$, $s=[1,1,0,0]$ and $t=[1,1,1,0,0,0,0]$,
we extend them to $\hat r=[1,1,0,0,0,0,0]$, $\hat s=[1,1,0,0,0,0,0]$ and $\hat t=t$,
which have the same length and consider the Recall measure of these new runs with common length equal to 7.
So from now on we consider to have a finite set of runs with fixed length, but evaluated with respect
to possible different Recall bases.
To explain how we proceed here let us start by an example. Let $r=[1,1,0,0,0]$; we have $Recall(5,2)[r]=2/2=1$ while
$Recall(5,3)[r]=2/3$. Thus the same judged run r can be evaluated by Recall in two different ways depending on the 
different values of the Recall base. So, denoting by $r_1$ the run for the topic with Recall base $2$ and
$r_2$ the run for the topic with Recall base $3$, we can embed these two runs as two runs for a topic with Recall base 
6 and length 6, where 6 is the Lowest Common Multiple of 2 and 3.
The transformed runs are $\hat r_1=[1,1,1,1,1,1]$ and $\hat r_2=[1,1,1,0,0,0]$, and it is immediate to see that 
$Recall(6,6)[\hat r_1]=Recall(5,2)[r_1]$ and $Recall(6,6)[\hat r_2]=Recall(5,3)[r_2]$.
Note that this embedding do not depends on the original lengths $N$ of the runs, but only on their Recall bases.
Thus, given a set of k runs, of same length $N$ and Recall bases, respectively, $RB_1, \ldots, RB_k$,
we denote by $\mathcal{RB}$ the Lowest Common Multiple of these Recall bases and extend the k runs
to k runs of same length equal to $\mathcal{RB}$ and such that their $Recall(\mathcal{RB},\mathcal{RB})$ is
equal to that of the original runs. The extended run $\hat r_i$ will have a number of relevant documents
equal to that of the original $r_i$ multiplied by $\mathcal{RB}/RB_i$ and a suitable additional number of not relevant documents
to arrive to the total length $\mathcal{RB}$.

It is important to point out that the two embedding developed for Precision and Recall are not compatible, and for this reason
the analysis of a set of runs evaluated by Precision and Recall are not equivalent. This can be seen by a simple example:
let $r=[1,1,0]$ and $s=[1,1,0,0]$ as in one of the previous examples. To consider them with Precision we 
transformed those as $\hat r=[1,1,1,1,1,1,1,1,0,0,0,0]$ and
$\hat s=[1,1,1,1,1,1,0,0,0,0,0,0]$, two runs of length 12, the Lowest Common Multiple of 3 and 4.
If we assume that the Recall base for the run $r$ is equal to 4 and that of $s$ equal to 3, respectively,
the transformation required to consider both the runs by the same Recall measure with Recall base equal to 12 leads to
$\tilde r=[1,1,1,1,1,1,0,0,0,0,0,0]=\hat s$ and
$\tilde s=[1,1,1,1,1,1,1,1,1,0,0,0]=\hat r$. So we get that the transformation leads to runs with the same lengths,
but switched. Thus the set of runs can be evaluated by the two
interval measures $Prec@12$ and $Recall(12,12)$ in a sound statistical way, but the two measures are not
equivalent and refer to different ordering amongst the runs, since for Precision $s$ is smaller then $r$ and for Recall $r$ is smaller than $s$.

\subsection{$F_1$ Measure}
The $F_1$ measure is the harmonic mean of precision and recall.
Its original definition for a run of length $N$ relative to a topic whose Recall base is $RB$, is
\[
F_1[r]=\frac{2}{(Prec@n[r])^{-1}+(Recall(N,RB)[r])^{-1}}
\]
Some small algebra making use of the definitions of $Prec@n$ and $Recall(N,RB)$ leads to the following, equivalent
definition
\begin{equation}
    \label{F1}
F_1[r]=\frac{2}{N+RB} \sum_{i=1}^N r [i]
\end{equation}
As before (see paper IEEE), we have that for fixed length and recall base, $F_1$ is an interval measure
equivalent to $Prec@n$ and $Recall(N,RB)$.

On the contrary, if we would like to analyse together runs of different lengths and/or relative to topics
with different recall bases, we can define a unique space of runs \& Recall bases where embed all the runs and evaluate
them with a unique measure. Inspired by the expression of (\ref{F1}), if we consider a family of runs
of lengths, respectively, $N_1,\ldots,N_k$ and relative to topic whose recall bases are $RB_1, \ldots, RB_k$,
we can first define $\mathcal{S}$ the Lowest Common Multiple of the set of numbers $N_1+RB_1,\ldots,N_k+RB_k$.
Let $L_i=\min(N_i,RB_i)$ and $\alpha_i=\mathcal{S}/(N_i+RB_i)$ for $i\in\{1,\ldots,k\}$: we have
\[
L_i\le\frac{N_i+RB_i}{2}= \frac{1}{2 \alpha_i} \mathcal{S} .
\]
If the run $r_i$ has $x_i$ relevant documents (and $N_i-x_i$ not relevant documents),
we make correspond to $r_i$ the run $\hat r_i$ of length $\lfloor \mathcal{S}\rfloor/2$ and relative to a
topic of recall base $\lfloor \mathcal{S} \rfloor/2$, with exactly $\alpha_i x_i$ relevant documents.
The $F_1$ score of $r_i$ is equal to the score 
\[
F_1[\hat r]=\frac{2}{\mathcal{S}} \sum_{i=1}^{\lfloor \mathcal{S} \rfloor/2} \hat r [i]
\]
and the embedding is well defined.

Let us apply this transformation to the example at the end of the previous sub section. Define again
$r=[1,1,0]$ and $s=[1,1,0,0]$ relative to topics with Recall bases, respectively, equal to 4 and to 3.
Since $N_1+RB_1=N_2+RB_2=7$, we get $\mathcal{S}=7$, $\lfloor \mathcal{S} \rfloor/2=3$
and the equivalent runs are $\hat r=[1,1,0]$ and $\hat s=[1,1,0]$.
To consider a more general situation, assume that the runs $r$ and $s$ are now 
relative to topics with Recall bases, respectively, equal to 3 and to 5.
Now $N_1+RB_1=6$ and $N_2+RB_2=9$ and we get $\mathcal{S}=18$, while $\lfloor \mathcal{S} \rfloor/2=9$.
The equivalent runs are here $\hat r=[1,1,1,1,1,1,0,0,0]$ and $\hat s=[1,1,1,1,0,0,0,0,0]$.

It is clear that the extended measure $F_1$ is interval for the family of the transformed runs, even if it is no more
a linear transformation of the interval equivalent to $Prec$ and $Recall$.

\subsection{$F_\beta$ Measure}
